Non-Parametric Modeling of Spatio-Temporal Human Activity Based on Mobile Robot Observations

This work presents a non-parametric spatio-temporal model for mapping human activity by mobile autonomous robots in a long-term context. Based on Variational Gaussian Process Regression, the model incorporates prior information of spatial and temporal-periodic dependencies to create a continuous representation of human occurrences. The inhomogeneous data distribution resulting from movements of the robot is included in the model via a heteroscedastic likelihood function and can be accounted for as predictive uncertainty. Using a sparse formulation, data sets over multiple weeks and several hundred square meters can be used for model creation. The experimental evaluation, based on multi-week data sets, demonstrates that the proposed approach outperforms the state of the art both in terms of predictive quality and subsequent path planning.

==> fig/paths_table_bck.tex <==
\begin{tabular}{ll>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.75cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.75cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.75cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.75cm}|>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.75cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.75cm}>{\raggedleft}p{0.6cm}>{\raggedleft}p{0.75cm}>{\raggedleft}p{0.6cm}>{\raggedleft\arraybackslash}p{0.75cm}}
\toprule
                                 &        & \multicolumn{8}{c|}{UoL-Office} & \multicolumn{8}{c|}{ATC} \\
                                 &        & \multicolumn{2}{c|}{{\scriptsize{\centering\arraybackslash}\parbox{1.7cm}{0.5\,m x 30\,min}}} & \multicolumn{2}{c|}{{\scriptsize{\centering\arraybackslash}\parbox{1.7cm}{0.5\,m x 60\,min}}} & \multicolumn{2}{c|}{{\scriptsize{\centering\arraybackslash}\parbox{1.7cm}{0.75\,m x 30\,min}}} & \multicolumn{2}{c|}{{\scriptsize{\centering\arraybackslash}\parbox{1.7cm}{0.75\,m x 60\,min}}} & \multicolumn{2}{c|}{{\scriptsize{\centering\arraybackslash}\parbox{1.7cm}{0.5\,m x 30\,min}}} & \multicolumn{2}{c|}{{\scriptsize{\centering\arraybackslash}\parbox{1.7cm}{0.5\,m x 60\,min}}} & \multicolumn{2}{c|}{{\scriptsize{\centering\arraybackslash}\parbox{1.7cm}{0.75\,m x 30\,min}}} & \multicolumn{2}{c|}{{\scriptsize{\centering\arraybackslash}\parbox{1.7cm}{0.75\,m x 60\,min}}} \\
                                 &        &                                                      {\scriptsize NRMSE} & {\scriptsize $\chi^2\mathrm{dst}$} &                                                      {\scriptsize NRMSE} & {\scriptsize $\chi^2\mathrm{dst}$} &                                                       {\scriptsize NRMSE} & {\scriptsize $\chi^2\mathrm{dst}$} &                                                       {\scriptsize NRMSE} & {\scriptsize $\chi^2\mathrm{dst}$} &                                                      {\scriptsize NRMSE} & {\scriptsize $\chi^2\mathrm{dst}$} &                                                      {\scriptsize NRMSE} & {\scriptsize $\chi^2\mathrm{dst}$} &                                                       {\scriptsize NRMSE} & {\scriptsize $\chi^2\mathrm{dst}$} &                                                       {\scriptsize NRMSE} & {\scriptsize $\chi^2\mathrm{dst}$} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{Static}} & ML &                                               2.66 &                   8.80 &                                               2.34 &                   8.01 &                                      \textbf{2.63} &                   8.66 &                                      \textbf{2.25} &                   7.73 &                                               2.66 &                   8.80 &                                               2.34 &                   8.01 &                                      \textbf{2.63} &                   8.66 &                                      \textbf{2.25} &                   7.73 \\
                                 & Fr-AAM &                                               2.71 &                   8.57 &                                                2.4 &                   7.82 &                                               2.76 &                   9.12 &                                               2.33 &                   8.07 &                                               2.71 &                   8.57 &                                                2.4 &                   7.82 &                                               2.76 &                   9.12 &                                               2.33 &                   8.07 \\
                                 & GP-Hom &                                               2.93 &                  10.60 &                                               2.66 &                  10.62 &                                               2.87 &                  10.43 &                                               2.53 &                  10.15 &                                               2.93 &                  10.60 &                                               2.66 &                  10.62 &                                               2.87 &                  10.43 &                                               2.53 &                  10.15 \\
                                 & GP-Het &                                      \textbf{2.59} &          \textbf{6.74} &                                      \textbf{2.33} &          \textbf{6.50} &                                               2.65 &          \textbf{6.95} &                                               2.32 &          \textbf{6.94} &                                      \textbf{2.59} &          \textbf{6.74} &                                      \textbf{2.33} &          \textbf{6.50} &                                               2.65 &          \textbf{6.95} &                                               2.32 &          \textbf{6.94} \\
\cline{1-18}
\multirow{4}{*}{\rotatebox[origin=c]{90}{Moving}} & ML &                                               2.61 &                  35.27 &                                               2.34 &                  32.03 &                                               2.57 &                  35.75 &                                               2.77 &                  38.89 &                                               2.61 &                  35.27 &                                               2.34 &                  32.03 &                                               2.57 &                  35.75 &                                               2.77 &                  38.89 \\
                                 & Fr-AAM &                                       \textbf{2.6} &         \textbf{33.72} &                                               2.38 &                  30.76 &                                               2.61 &                  33.89 &                                               2.67 &                  34.89 &                                       \textbf{2.6} &         \textbf{33.72} &                                               2.38 &                  30.76 &                                               2.61 &                  33.89 &                                               2.67 &                  34.89 \\
                                 & GP-Hom &                                               2.76 &                  46.18 &                                                2.8 &                  44.18 &                                               2.91 &                  44.56 &                                               3.22 &                  54.88 &                                               2.76 &                  46.18 &                                                2.8 &                  44.18 &                                               2.91 &                  44.56 &                                               3.22 &                  54.88 \\
                                 & GP-Het &                                               2.61 &                  50.52 &                                      \textbf{2.13} &         \textbf{24.91} &                                      \textbf{2.33} &         \textbf{25.28} &                                      \textbf{2.19} &         \textbf{25.20} &                                               2.61 &                  50.52 &                                      \textbf{2.13} &         \textbf{24.91} &                                      \textbf{2.33} &         \textbf{25.28} &                                      \textbf{2.19} &         \textbf{25.20} \\
\bottomrule
\end{tabular}

